Effective Embedding of Integer Linear Inequalities for Variational Quantum Algorithms

In variational quantum algorithms, constraints are usually added to the problem objective via penalty terms. For linear inequality constraints, this procedure requires additional slack qubits. Those extra qubits tend to blow up the search space and complicate the parameter landscapes to be navigated by the classical optimizers. In this work, we explore approaches to model linear inequalities for quantum algorithms without these drawbacks. More concretely, our main suggestion is to omit the slack qubits completely and evaluate the inequality classically during parameter tuning. We test our methods on QAOA as well as on Trotterized adiabatic evolution, and present empirical results. As a benchmark problem, we consider different instances of the multi-knapsack problem. Our results show that removing the slack bits from the circuit Hamiltonian and considering them only for the expectation value yields better solution quality than the standard approach. The tests have been carried out using problem sizes up to 26 qubits. Our methods can in principle be applied to any problem with linear inequality constraints, and are suitable for variational as well as digitized versions of adiabatic quantum computing.

==> Sections/Apdx_alpha_hamiltonian.tex <==
\section{Including the knapsack's filling level as a parameter in the quantum circuit (old $\alpha$-QAOA idea)}

\subsection{Hybrid QUBO Formulation}

1) Any item $i$ can be assigned to a maximum one knapsack. It is possible that an item is not assigned to any knapsack

\begin{equation}
\small
H_{\text{single}}= \sum_{j=0}^{N-1} \left(\sum_{i=0}^{M-1} x_{i,j}\right)\cdot \left(\sum_{i=0}^{M-1} x_{i,j}-1 \right) \;.
\end{equation}

2) Ensure that the capacity of any knapsack is not exceeded. This is achieved by incorporating a positive continuous variable $\alpha_i$ for each knapsack $i$, as shown below. 

\begin{equation}
\small
\text{H}_{\text{capacity}}^{\alpha}=\sum_{i=0}^{M-1} \left[\left(\sum_{j=0}^{N-1} w_j\cdot x_{i,j}\right) + \alpha_i - c_i \right]^2 \;.
\end{equation}


\begin{equation}
\small
	H_{\text{capacity}}^{\alpha}=\sum_{i=0}^{M-1} \left[\left(\sum_{j=0}^{N-1} w_j\cdot x_{i,j}\right) - c_i \right]^2 + \sum_{i=0}^{M-1} \left( \alpha_i^2 + \sum_{j=0}^{N-1}2w_j\alpha_i x_{i,j} -2\alpha_i C_i \right) . 
\end{equation}

\begin{equation}
\small
	H_{\text{capacity}}^{\alpha}= \text{QUBO}(x_{i,j},w_j, c_i) + \sum_{i=0}^{M-1} \left( \alpha_i^2 + \sum_{j=0}^{N-1}2w_j\alpha_i x_{i,j} -2\alpha_i c_i \right) . 
\end{equation}


\begin{equation}
\small
	H_{\text{capacity}}^{\alpha}= \text{QUBO}(x_{i,j},w_j, c_i) + \sum_{i=0}^{M-1} \sum_{j=0}^{N-1}2w_j\alpha_i x_{i,j}  + \sum_{i=0}^{M-1} \left( \alpha_i^2 - 2\alpha_i c_i \right) \;. 
\end{equation}


The fact that $w_j$ $\forall j$ and $c_i$ $\forall i$ are positive integers, a feasible solution for $H_{\text{capacity}}^{\alpha}$ will ensure that $\alpha_i\in\mathbb{N}^{+}$ $\forall i$.

3) Maximize the total value of assigned items in knapsacks

\begin{equation}
\small
H_{\text{obj}}= - \sum_{i=0}^{M-1} \sum_{j=0}^{N-1} v_{i,j} \cdot x_{i,j} \;.
\end{equation}

Finally, the complete QUBO is written as,

\begin{equation}
\small
H^{\alpha} = A\cdot H_{\text{single}} + B\cdot \text{H}_{\text{capacity}}^{\alpha} + C \cdot H_{\text{obj}} \;, \\
\end{equation}

where $A,B $ are the penalty coefficients, and $C$ is the objective weight. Note, $A>0, B>0, C >0$. The above QUBO $H^{\alpha}$ is a QUBO formulation for the multi-knapsack problem parameterized with continuous variable $\alpha_i$. We propose to optimize $\alpha_i$s using the classical optimizers in quantum variational ansatz. 

Since the QAOA works with the parametric unitarization of the Ising model, we first transform the $H_{\text{capacity}}^{\alpha}$ to the Ising model by substituting $x$ with $(1-x)/2$, such that

\begin{equation}
\small
	H_{\text{capacity}}^{\alpha,(\text{ising})}= \text{ISING}(x_{i,j},w_j, c_i) - \sum_{i=0}^{M-1} \sum_{j=0}^{N-1}w_j\alpha_i x_{i,j} +\sum_{i=0}^{M-1}\left( \alpha_i^2 + \sum_{j=0}^{N-1}w_j\alpha_i -2\alpha_i c_i \right) \;. 
\end{equation}

With the help of the above equation we can easily build the required quantum circuit for $H_{\text{capacity}}^{\alpha,(\text{ising})}$ by inserting an additional unitary operator $\exp\left(-i\gamma (- \sum_{i=0}^{M-1} \sum_{j=0}^{N-1}w_j\alpha_i x_{i,j})\right)$, with $0\leq \alpha_i \leq c_i $ and $\gamma\in[0, 2\pi]$, $\forall i,j$.

As for the $\alpha$ dependent offset term in $H_{\text{capacity}}^{\alpha,(\text{ising})}$, we neglect it for the QAOA quantum circuit, but consider it in the computation of the expectation value of the sampled quantum states. The reason for neglecting this offset term is the fact that it does not depend on the quantum states and is optimized only by the classical solvers which are also responsible for optimizing $\beta$ and $\gamma$ angles.

